Quantum Fourier Networks for Solving Parametric PDEs

Many real-world problems, like modelling environment dynamics, physical processes, time series etc., involve solving Partial Differential Equations (PDEs) parameterised by problem-specific conditions. Recently, a deep learning architecture called Fourier Neural Operator (FNO) proved to be capable of learning solutions of given PDE families for any initial conditions as input. However, it results in a time complexity linear in the number of evaluations of the PDEs while testing. Given the advancements in quantum hardware and the recent results in quantum machine learning methods, we exploit the running efficiency offered by these and propose quantum algorithms inspired by the classical FNO, which result in time complexity logarithmic in the number of evaluations and are, therefore, expected to be substantially faster than their classical counterpart. At their core, we use the unary encoding paradigm and orthogonal quantum layers and introduce a circuit to perform quantum Fourier transform in the unary basis. We propose three different quantum circuits to perform a quantum FNO. The proposals differ in their depth and their similarity to the classical FNO. We also benchmark our proposed algorithms on three PDE families, namely Burgers' equation, Darcy's flow equation and the Navier-Stokes equation. The results show that our quantum methods are comparable in performance to the classical FNO. We also perform an analysis on small-scale image classification tasks where our proposed algorithms are at par with the performance of classical CNNs, proving their applicability to other domains as well.

==> fig_1.tex <==
\begin{figure*}[!ht]
    \begin{subfigure}[t]{0.33\textwidth}
    \begin{tikzpicture}
    \begin{axis}[
        title = {$\QAOA$ depth, $p = \frac{3n}{4}$},
        xlabel={No. qubits},
        ylabel={Approximation ratio, $r$},
        ylabel near ticks,
        legend cell align={left},
        xmin=3, xmax=17,
        ymin=0.65, ymax= 1.02,
        xtick={ 4, 6, 8, 10, 12, 14, 16},
        ytick={0.6, 0.65, 0.70, 0.75, 0.80, 0.85, 0.90, 0.95, 1.00},
        legend pos=south west,
        ymajorgrids=true,
        grid   = major,
        height = 5.2cm,
        width  = 5.65cm
    ]
    \addplot[
        color=blue,
        mark=square*,
        ]
        coordinates {
     (4,   0.94)
     (6,   0.92)
     (8,   0.93)
     (10,   0.94)
     (12,   0.89)
     (14,   0.88)
     (16,   0.89)
    };
 
    \addplot[
        color=magenta,
        mark=triangle*,
        ]
        coordinates {
     (4,   1)
     (6,  0.99)
     (8,   0.99)
     (10,   0.98)
     (12,   0.967)
     (14,   0.97)
     (16,   0.96)
    };
    \addplot[
        color=green,
        mark=triangle*,
        ]
        coordinates {
     (4,   1)
     (6,  0.95)
     (8,   0.96)
     (10,   0.96)
     (12,   0.95)
     (14,   0.95)
     (16,   0.94)
    };
    \addplot[
        color=red,
        mark=diamond*,
        ]
        coordinates {
     (4,   0.92)
     (6,  0.94)
     (8,   0.94)
     (10,   0.95)
     (12,   0.94)
     (14,   0.93)
     (16,   0.91)
    };
    \legend{LGNN, LGNN $\QAOA$, GCN $\QAOA$ , Cold-start $\QAOA$}
    \end{axis}
    \end{tikzpicture}
    \caption{}
    \label{fig:gnn_maxcut_scores_a}
    \end{subfigure}
    %
      \begin{subfigure}[t]{0.3\textwidth}
    \begin{tikzpicture}
    \begin{axis}[
        title = {$\QAOA$ depth, $p = \frac{n}{2}$},
        xlabel={No. qubits},
        ylabel={},
        ylabel near ticks,   
        % yticklabels={,,},
        legend cell align={left},
        xmin=3, xmax=17,
        ymin=0.65, ymax= 1.02,
        xtick={ 4, 6, 8, 10, 12, 14, 16},
        ytick={0.6, 0.65, 0.70, 0.75, 0.80, 0.85, 0.90, 0.95, 1.00},
        legend pos=south west,
        ymajorgrids=true,
        grid   = major,
        height = 5.2cm,
        width  = 5.8cm
    ]
    \addplot[
        color=blue,
        mark=square*,
        ]
        coordinates {
     (4,   0.94)
     (6,   0.92)
     (8,   0.93)
     (10,   0.94)
     (12,   0.89)
     (14,   0.88)
     (16,   0.89)
    };
    \addplot[
        color=magenta,
        mark=triangle*,
        ]
        coordinates {
     (4,   0.96)
     (6,  0.95)
     (8,   0.93)
     (10,   0.97)
     (12,   0.94)
     (14,   0.93)
     (16,   0.95)
    };
    \addplot[
        color=green,
        mark=*,
        ]
        coordinates {
     (4,   0.93)
     (6,  0.92)
     (8,   0.91)
     (10,   0.94)
     (12,   0.92)
     (14,   0.91)
     (16,   0.92)
    };
    \addplot[
        color=red,
        mark=diamond*,
        ]
        coordinates {
     (4,   0.79)
     (6,  0.81)
     (8,   0.84)
     (10,   0.82)
     (12,   0.83)
     (14,   0.88)
     (16,   0.90)
    };
    % \legend{LGNN, LGNN $\QAOA$, GCN $\QAOA$, Cold-start $\QAOA$}
    \end{axis}
    \end{tikzpicture}
    \caption{}
    \label{fig:gnn_maxcut_scores_b}
    \end{subfigure}
    %
        %
      \begin{subfigure}[t]{0.3\textwidth}
    \begin{tikzpicture}
    \begin{axis}[
        title = {No. qubits $=16$},
        xlabel={$\QAOA$ depth, $p$},
        ylabel={},
        ylabel near ticks,   %yticklabels={,,},
        legend cell align={left},
        xmin= 0.5, xmax=10.5,
        ymin=0.45, ymax= 1.02,
        xtick={ 1, 2, 3, 4,5,6,7,8,9, 10},
        % ytick={0.4, 0.5, 0.55, 0.6, 0.65, 0.70, 0.75, 0.80, 0.85, 0.90, 0.95, 1.00},
        ytick={0.4, 0.5, 0.6,0.70,  0.80,  0.90,  1.00},
        legend pos=south west,
        ymajorgrids=true,
        grid   = major,
        height = 5.2cm,
        width  = 5.8cm
    ]
    % \addplot[
    %     color=blue,
    %     mark=square*,
    %     ]
    %     coordinates {
    %  (4,   0.94)
    %  (6,   0.92)
    %  (8,   0.93)
    %  (10,   0.94)
    %  (12,   0.89)
    %  (14,   0.88)
    %  (16,   0.89)
    % };
    \addplot[
        color=magenta,
        mark=triangle*,
        ]
        coordinates {
     (1,   0.72)
     (2,  0.85)
     (3,   0.87)
     (4,   0.89)
     (5,   0.92)
     (6,   0.93)
     (7,   0.94)
     (8,   0.95)
     (9,   0.98)
     (10,   0.98)
    };
    \addplot[
        color=green,
        mark=*,
        ]
        coordinates {
     (1,   0.67)
     (2,  0.79)
     (3,   0.84)
     (4,   0.87)
     (5,   0.90)
     (6,   0.90)
     (7,   0.91)
     (8,   0.92)
     (9,   0.96)
     (10,   0.98)
    };
    \addplot[
        color=red,
        mark=diamond*,
        ]
        coordinates {
     (1,   0.47)
     (2,  0.58)
     (3,   0.67)
     (4,   0.74)
     (5,   0.79)
     (6,   0.85)
     (7,   0.88)
     (8,   0.90)
     (9,   0.93)
     (10,   0.96)
    };
    % \legend{LGNN, LGNN $\QAOA$, GCN $\QAOA$, Cold-start $\QAOA$}
    \end{axis}
    \end{tikzpicture}
    \caption{}
    \label{fig:gnn_maxcut_scores_c}
    \end{subfigure}
\caption{\textbf{Performance of the graph neural network on $3$-regular graphs for $\maxcut$.} We compare the $\maxcut$ approximation ratios achieved with LGNN/GCN initialisation versus cold-start (vanilla) $\QAOA$. We also plot the raw values outputted by the LGNN with a simple rounding scheme. In (a), the $\QAOA$ depth is set to be $p=3n/4$, while in (b), $p=n/2$. Each datapoint is generated via $1000$ runs of the LGNN/GCN on random instances of $3$-regular graphs, of the appropriate size to the number of qubits. Finally, in (c), we fix the number of qubits to be $16$ and plot each method as a function of the $\QAOA$ depth, demonstrating monotonic improvement as a function of $p$. Each datapoint is generated via $1000$ runs of the LGNN/GCN on random instances of $3$-regular graphs, of the appropriate size to the number of qubits.}
\label{fig:gnn_maxcut_numerics}
\end{figure*}


